Faithfulness Measurable Masked Language Models

A common approach to explaining NLP models is to use importance measures that express which tokens are important for a prediction. Unfortunately, such explanations are often wrong despite being persuasive. Therefore, it is essential to measure their faithfulness. One such metric is if tokens are truly important, then masking them should result in worse model performance. However, token masking introduces out-of-distribution issues, and existing solutions that address this are computationally expensive and employ proxy models. Furthermore, other metrics are very limited in scope. This work proposes an inherently faithfulness measurable model that addresses these challenges. This is achieved using a novel fine-tuning method that incorporates masking, such that masking tokens become in-distribution by design. This differs from existing approaches, which are completely model-agnostic but are inapplicable in practice. We demonstrate the generality of our approach by applying it to 16 different datasets and validate it using statistical in-distribution tests. The faithfulness is then measured with 9 different importance measures. Because masking is in-distribution, importance measures that themselves use masking become consistently more faithful. Additionally, because the model makes faithfulness cheap to measure, we can optimize explanations towards maximal faithfulness; thus, our model becomes indirectly inherently explainable.

==> chapter/ethics.tex <==
% Scientific work published at EMNLP 2023 must comply with the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL Ethics Policy}. We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).
\section*{Ethics Statement}
Interpretability is an essential component when considering the ethical deployment of a model. In this paper, we particularly consider deployment a key motivator in our work, as we specify that for a \emph{faithfulness measurable model} the deployed model and measured model should be the same. Without this criterion, there is a dangerous potential for discrepancies between the analyzed model and the deployed model.

However, there is still a risk that the faithfulness measure itself can be wrong. This is problematic, as a false faithfulness measure would create unjustified confidence in the importance measure. A key assumption with our proposed metric is that the model provides in-distribution support for any permutation of masked tokens. We take extra care to validate this assumption using sound methodologies. Note that our work is not the only one with this assumption, in particular ROAR-based metrics \citep{Hooker2019, Madsen2022} assume in-distribution behavior, but do not test for this. Additionally, we attempt to provide complete transparency regarding all the limitations of our faithfulness metric.

\subsection*{Use of anonymized medical data}
The Diabetes and Anemia datasets used in this work are based on the anonymized open-access medical database MIMIC-III \citep{Johnson2016}. These datasets are used because they are common in the faithfulness literature \citep{Jain2019, Madsen2022}. In particular, they contain many redundancies and are long-sequence datasets. The specific authors of this paper, who have worked with this data, have undergone the necessary HIPAA certification in order to access this data and comply with HIPAA regulations.

